SymmetryNet: Learning to Predict Reflectional and Rotational Symmetries of 3D Shapes from Single-View RGB-D Images

We study the problem of symmetry detection of 3D shapes from single-view RGB-D images, where severely missing data renders geometric detection approach infeasible. We propose an end-to-end deep neural network which is able to predict both reflectional and rotational symmetries of 3D objects present in the input RGB-D image. Directly training a deep model for symmetry prediction, however, can quickly run into the issue of overfitting. We adopt a multi-task learning approach. Aside from symmetry axis prediction, our network is also trained to predict symmetry correspondences. In particular, given the 3D points present in the RGB-D image, our network outputs for each 3D point its symmetric counterpart corresponding to a specific predicted symmetry. In addition, our network is able to detect for a given shape multiple symmetries of different types. We also contribute a benchmark of 3D symmetry detection based on single-view RGB-D images. Extensive evaluation on the benchmark demonstrates the strong generalization ability of our method, in terms of high accuracy of both symmetry axis prediction and counterpart estimation. In particular, our method is robust in handling unseen object instances with large variation in shape, multi-symmetry composition, as well as novel object categories.

==> embedding.tex <==
%!TEX root = sceneparse.tex

\subsection{Symmetry-aware point feature embedding}
\label{sec:embedding}

Since the input contains both RGB images and depth images, the first question to be addressed is how to fuse the features from the two modalities.
%There are a variety number of works that could used to this task
While a variety of methods can be used for this task, we follow the approach described in [densefusion] to solve this problem. Specifically, the approach in [densefusion] extracts per-point appearance feature and geometry feature via a fully-convolutional network [?] and a PointNet [pointnet], respectively.
The two kinds of features are then concatenated and used for pixel-wise prediction tasks.

To make the features relevant to object symmetry, we propose to learn a symmetry-aware point feature embedding in which the symmetric counterparts have similar features. This is achieved by using a triplet loss [?]:
\begin{equation}\label{eq:triplet_focal_loss}
  L_{embed}(f_a,f_p,f_n) = \max \bigl(0, \alpha - [d(f_n, f_a) - d(f_p, f_a)]\bigr),
\end{equation}
where $f_a$, $f_p$ and $f_n$ are the feature vectors extracted for the anchor, the positive, and the negative points, respectively, and $d$ is the Euclidean distance between two specific features. $\alpha$ is a pre-defined threshold.

The training data of this network is collected from large scale 3D object datasets with ground-truth symmetry labels.
For training data preparation, we first select anchor points and take their counterpart as positives. The negatives are any of the non-counterpart points. The anchor points whose counterparts are not visible in the RGB-D image are not selected.
In our experiment, we found that the strategy of randomly selecting negatives leads to fast converge during the training procedure, due to the fact that most of the negatives can be easily distinguished. As a consequence, the training becomes less efficient.

%\ys{
We opt to use an offline hard negative mining to collect hard samples.
%Firstly, instead of randomly selecting the anchor points, we ?.
We first compute SIFT feature [?] and Fast Point Feature Histograms (FPFH) descriptor [?] for the input RGB image and depth image, respectively.
To generate quality negative data, we select non-counterpart points whose SIFT feature and FPFH descriptor are closed to those of the anchor points in the feature spaces.
Such hard negative data enables the network to better understand how the points match w.r.t the symmetries, ensuring efficient training of the predicion network.
Figure ? visualizes the feature embedding trained by the triplet loss.
%}


==> overview.tex <==
%!TEX root = sceneparse.tex

\section{Overview}
\label{sec:overview}

